Overcoming Distribution Mismatch in Quantizing Image Super-Resolution Networks

Although quantization has emerged as a promising approach to reducing computational complexity across various high-level vision tasks, it inevitably leads to accuracy loss in image super-resolution (SR) networks. This is due to the significantly divergent feature distributions across different channels and input images of the SR networks, which complicates the selection of a fixed quantization range. Existing works address this distribution mismatch problem by dynamically adapting quantization ranges to the varying distributions during test time. However, such a dynamic adaptation incurs additional computational costs during inference. In contrast, we propose a new quantization-aware training scheme that effectively Overcomes the Distribution Mismatch problem in SR networks without the need for dynamic adaptation. Intuitively, this mismatch can be mitigated by regularizing the distance between the feature and a fixed quantization range. However, we observe that such regularization can conflict with the reconstruction loss during training, negatively impacting SR accuracy. Therefore, we opt to regularize the mismatch only when the gradients of the regularization are aligned with those of the reconstruction loss. Additionally, we introduce a layer-wise weight clipping correction scheme to determine a more suitable quantization range for layer-wise weights. Experimental results demonstrate that our framework effectively reduces the distribution mismatch and achieves state-of-the-art performance with minimal computational overhead.

==> sections/figures/exp-loss.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure_files/dist.pdf}
        % \fbox{\rule[-.5cm]{0cm}{3cm} \rule[-.5cm]{3cm}{0cm}}
        \caption{EDSR \label{fig:exp-loss-a}}
    \end{subfigure} 
    % \hfill
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure_files/dist.pdf}
        % \fbox{\rule[-.5cm]{0cm}{3cm} \rule[-.5cm]{3cm}{0cm}}
        \caption{SRResNet \label{fig:exp-loss-b}}
    \end{subfigure}
    \caption{ 
        % The effect of our framework on average mismatch during training. 
        The average distribution mismatch curve during training. Distribution mismatch is measured by summing the feature variance for all quantized convolutional features.
        \cheeun{maybe this isn't necessary}
    }
    \label{fig:exp-loss}
\end{figure}

==> sections/figures/method-location.tex <==
\begin{figure}[t]
    \begin{subfigure}{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure_files/loc1.pdf}
        % \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
        \caption{Existing quantization location \label{fig:method-location-a}}
    \end{subfigure} 
    \hfill
    \begin{subfigure}{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure_files/loc2.pdf}
        % \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
        \caption{Our quantization location \label{fig:method-location-b}}
    \end{subfigure}
    \caption{ 
        \textbf{location} write caption here
    }
    \label{fig:method-location}
\end{figure}

==> sections/figures/method-motivation.tex <==
\begin{figure}[t]
    \centering
    \newcommand{\w}{0.3\textwidth}
    \begin{subfigure}{\w}
        \centering
        \includegraphics[width=\textwidth]{figure_files/featuremap-channel_blk3_sample5_2_good.pdf}
        \caption{
            Small distribution mismatch
            % $M_w$: \textcolor{red}{Low}, $M_b$: \textcolor{red}{Low} 
            \label{fig:method-offset-a}
        }
    \end{subfigure}
    \hfill
    \begin{subfigure}{\w}
        \centering
        \includegraphics[width=\textwidth]{figure_files/featuremap-channel_blk4_sample2_2_good.pdf}
        \caption{
            Mismatch in channel-wise $\sigma$
            % $M_w$: \textcolor{blue}{High}, $M_b$: \textcolor{red}{Low}
            \label{fig:method-offset-b}
        }
    \end{subfigure} 
    \hfill
    \begin{subfigure}{\w}
        \centering
        \includegraphics[width=\textwidth]{figure_files/featuremap-channel_blk12_sample2_2_good.pdf}
        \caption{
            % $M_w$: \textcolor{red}{Low}, $M_b$: \textcolor{blue}{High} 
            Mismatch in channel-wise $\mu$
            \label{fig:method-offset-c}
        }
    \end{subfigure}
    \vspace{-0.2cm}
    \caption{
        \textbf{The distribution mismatch of different layers in EDSR.}
        While layer (a) shows an overall small mismatch between channels, layer (b) shows a large mismatch on deviation, and layer (c) exhibits a large mismatch on average. 
        This motivates us to selectively \textit{scale} features with large deviation mismatch ($\vm^\sigma$) and \textit{shift} features with a large average mismatch ($\vm^\mu$). 
    }
    \vspace{-0.2cm}
    \label{fig:method-offset}
\end{figure}

==> sections/figures_sup/sup-obs.tex <==
\begin{figure}[!h]
\centering
% \includegraphics[width=0.98\textwidth]{figure_files/mismatch3.pdf}
    \subfloat[Channel-wise features]{
        \includegraphics[width=0.4\textwidth]{figure_files/variance_ch2.pdf}
    }
    \subfloat[Image-wise features]{
        \includegraphics[width=0.4\textwidth]{figure_files/variance_img2.pdf}
    }
% \vspace{-0.2cm}
\caption{
    \textbf{Distribution mismatch in SR networks.} 
    % Compared to an classification network (\eg, ResNet-18), the SR network (\eg, EDSR) exhibits a large mismatch inside the feature distributions in channel and image dimensions.
    % The large distribution mismatch causes difficulties in selecting an appropriate quantization range.
    Channel-wise and image-wise features of different layers of EDSR are visualized.
    The visualized channels and images are randomly selected.
    % Channels and images of the 2nd conv layer of EDSR are randomly selected for visualization.
    % Additional results are provided in the supplementary material.
}
\label{fig:sup-obs}
% \vspace{-0.2cm}
\end{figure}



==> sections/figures_sup/sup-qual.tex <==
\begin{figure}[h]
\centering
\begin{center}
    \setlength{\tabcolsep}{0.07cm}
    \newcommand{\w}{0.18\linewidth}
    \begin{tabular}{ccccc}
        \centering
        % \includegraphics[width=\w]{figure_files/qual/barbara_GT.png} &
        \includegraphics[width=\w]{figure_files/qual/img060_GT.png} &
        \includegraphics[width=\w]{figure_files/qual/img060_pamsf.png} &
        \includegraphics[width=\w]{figure_files/qual/img060_daq.png} &
        \includegraphics[width=\w]{figure_files/qual/img060_ddtb.png} &
        \includegraphics[width=\w]{figure_files/qual/img060_ours.png} \\
        % \small GT &\small EDSR~\cite{lim2017enhanced} &\small EDSR-PAMS &\small EDSR-DAQ &\small EDSR-DDTB &\small EDSR-ODM \\
        % \small GT (img060) &\small EDSR-DAQ &\small EDSR-DDTB &\small EDSR-ODM \\
        \small GT (img060) & \small EDSR-PAMS & \small EDSR-DAQ &\small EDSR-DDTB &\small \textbf{EDSR-ODM} \\
        % \vspace{5mm}
        \\
        % \includegraphics[width=\w]{figure_files/qualitative results/1215_30_crop_GT.png} &
        \includegraphics[width=\w]{figure_files/qual/img004_GT.png} &
        \includegraphics[width=\w]{figure_files/qual/img004_pamsf.png} &
        \includegraphics[width=\w]{figure_files/qual/img004_daq.png} &
        \includegraphics[width=\w]{figure_files/qual/img004_ddtb.png} &
        \includegraphics[width=\w]{figure_files/qual/img004_ours.png} \\
        % \small GT & \small SRResNet~\cite{ledig2017photo} &\small SRResNet-PAMS &\small SRResNet-DAQ &\small SRResNet-DDTB &\small SRResNet-ODM 
        \small GT (img004) & \small RDN-PAMS &\small RDN-DAQ &\small RDN-DDTB &\small \textbf{RDN-ODM} \\
        \\
        \includegraphics[width=\w]{figure_files/qual/img048_GT.png} &
        \includegraphics[width=\w]{figure_files/qual/img048_pamsf.png} &
        \includegraphics[width=\w]{figure_files/qual/img048_daq.png} &
        \includegraphics[width=\w]{figure_files/qual/img048_ddtb.png} &
        \includegraphics[width=\w]{figure_files/qual/img048_ours.png} \\
        % \small GT & \small SRResNet~\cite{ledig2017photo} &\small SRResNet-PAMS &\small SRResNet-DAQ &\small SRResNet-DDTB &\small SRResNet-ODM 
        \small GT (img048) & \small SRResNet-PAMS &\small SRResNet-DAQ &\small SRResNet-DDTB &\small \textbf{SRResNet-ODM} 
        \\
    \end{tabular}
    \caption{
    \textbf{Qualitative results} on EDSR, RDN, and SRResNet of scale 4. 
    }
    \label{fig:sup-qual}
\end{center}
\end{figure}




==> sections/tables/exp-srresnet.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{1.2mm}
\caption{ \textbf{Quantitative comparisons on SRResNet} of scale 4.
% IDN~\cite{hui2018idn}, EDSR-baseline~\cite{lim2017enhanced}, SRResNet, and CARN~\cite{ahn2018fast} of scale 4.
% The average feature quantization rate of the feature extraction stage (FQR), PSNR, and SSIM are reported.
% The results demonstrate the efficiency of the proposed method that manages to reduce FQR while maintaining or improving PSNR/SSIM
% \vspace{-2mm}
\vspace{-0.2cm}
}
% Turquoise / YellowGreen / Emerald / Orchid
% \resizebox{\textwidth}{!}{
\scalebox{0.85}{
    \begin{tabular}{l c cc cc cc cc}
        \toprule
        \multirow{2}{*}{Model} & \multirow{2}{*}{Bit} & 
        \multicolumn{2}{c}{Set5} & \multicolumn{2}{c}{Set14} & \multicolumn{2}{c}{B100} & \multicolumn{2}{c}{Urban100} \\
        \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}& 
         & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM \\
        \midrule 
        SRResNet   &32 &32.07&0.893 &28.50&0.780 &27.52&0.735 &25.86&0.779\\
        \midrule
        SRResNet-PAMS   &4  &31.88&0.891 &28.41&0.777 &27.45&0.732 &25.68&0.773\\
        SRResNet-DAQ   &4  &31.85&0.889 &28.41&0.777 &27.45&0.732 &25.70&0.772\\
        SRResNet-DDTB&4  &31.97&0.892 &28.46&0.778 &27.48&0.733 &25.77&0.776\\
        % SRResNet-QuantSR&4  &31.97&0.892 &28.46&0.778 &27.48&0.733 &25.77&0.776\\
        \rowcolor{YellowGreen!25}
        SRResNet-ODM (Ours)              &4 & \textbf{32.00}&\textbf{0.892} &\textbf{28.46}&\textbf{0.778} &\textbf{27.48}&\textbf{0.734} &\textbf{25.77}&\textbf{0.776} \\
        \midrule
        SRResNet-PAMS   &3 &31.68&0.888 &28.27&0.774 &26.79&0.709 &25.46&0.765\\
        SRResNet-DAQ   &3 &31.81&0.889 &28.35&0.776 &27.40&0.733 &25.63&0.772\\
        SRResNet-DDTB&3 &31.85&0.890 &28.39&0.776 &27.44&0.731 &25.64&0.770\\
        \rowcolor{YellowGreen!25}
        SRResNet-ODM (Ours)              &3 &\textbf{31.86}&\textbf{0.890} &\textbf{28.39}&\textbf{0.776} &\textbf{27.44}&\textbf{0.732} &\textbf{25.65}&\textbf{0.771}\\
        \midrule
        SRResNet-PAMS   &2 &30.25&0.861 &27.36&0.750 &26.79&0.709 &24.19&0.713\\
        SRResNet-DAQ   &2 &31.57&0.886 &28.19&0.773 &27.30&0.729 &25.39&0.765\\
        % SRResNet-DAQ   &2 &31.67&0.000 &28.26&0.000 &27.32&0.000 &25.39&0.000\\
        SRResNet-DDTB&2 &31.51&0.887 &28.23&0.773 &27.33&0.728 &25.37&0.762\\
        % SRResNet-QuantSR&2 &31.30&0.88? &28.23&0.773 &27.33&0.728 &25.37&0.762\\
        % \rowcolor{cyan!15}
        \rowcolor{YellowGreen!25}
        SRResNet-ODM (Ours)              &2 &\textbf{31.59}&\textbf{0.887} &\textbf{28.27}&\textbf{0.773} &\textbf{27.36}&\textbf{0.729} &\textbf{25.44}&\textbf{0.765}\\
        \bottomrule
    \end{tabular}
}
% \vspace{-0.2cm}
\label{tab:exp-srresnet}
\end{table}




==> sections/tables/intro-mismatch.tex <==
\begin{table}[!t]
    \centering
    \setlength{\tabcolsep}{1.3mm}
    \caption{
    \textbf{Average feature mismatch} on image super-resolution networks (EDSR and RDN) and image classification network (ResNet-20). The metrics are measured on DIV2K validation set for SR networks and ImageNet validation set for the classification network.
    \cheeun{should change this to avg QE? for both weight and activation? or maybe change this into fig??? also, should use the same dataset (div2k val set) for inputs.}
    \cheeun{or change to swinir instead of rdn?}
    \cheeun{key: mismatch is more severe for SR than other tasks}
    } 
    % 똑같이 맞춰주기? to ImageNet validation set?
    \resizebox{0.9\linewidth}{!}{
            \begin{tabular}{llc ccc}
                \toprule
                Task & Model & Image-wise Variance & Channel-wise Variance \\
                \midrule
                Image super-resolution & EDSR ($\times4$) & 15.08 & 40.29\\
                Image super-resolution & RDN ($\times4$) & 6.40 & 58.14 \\
                Image classification & ResNet-20 & 0.04 & 0.09\\
                \bottomrule
            \end{tabular}
    }
    % \label{tab:sup-analyses-mismatch}
    \label{tab:intro-mismatch}
\end{table}
